The geometry of the moduli Space of non-cyclic biquadratic field extensions

In this paper, we investigate the existence of an elementary abelian closure in characteristic not $2$ for biquadratic extensions. We discover that it exists for any non-cyclic extension. We make use of it to obtain a classification for this class of extensions up to isomorphism via descent. This permits us to describe the geometry of this moduli space in group theoretic terms. We also provide two families of polynomials with two parameters that can describe any quartic extensions.

==> introduction.tex <==

In this paper we classify all non-cyclic biquadratic field extension up to isomorphism, this works extends the work
done by S. Marques and K. Ward in \cite{cubic}
